Accurate waveform models for gravitational-wave astrophysics: synergetic approaches from analytical relativity

Gravitational-wave (GW) astrophysics is a field in full blossom. Since the landmark detection of GWs from a binary black hole on September 14th 2015, several compact-object binaries have been reported by the LIGO-Virgo collaboration. Such events carry astrophysical and cosmological information ranging from an understanding of how black holes and neutron stars are formed, what neutron stars are composed of, how the Universe expands, and allow testing general relativity in the highly-dynamical strong-field regime. It is the goal of GW astrophysics to extract such information as accurately as possible. Yet, this is only possible if the tools and technology used to detect and analyze GWs are advanced enough. A key aspect of GW searches are waveform models, which encapsulate our best predictions for the gravitational radiation under a certain set of parameters, and that need to be cross-correlated with data to extract GW signals. Waveforms must be very accurate to avoid missing important physics in the data, which might be the key to answer the fundamental questions of GW astrophysics. The continuous improvements of the current LIGO-Virgo detectors, the development of next-generation ground-based detectors such as the Einstein Telescope or the Cosmic Explorer, as well as the development of the Laser Interferometer Space Antenna (LISA), demand accurate waveform models. [Abridged.]

==> intro/acknowledgements.tex <==
\begin{center}
    \textbf{Acknowledgements}
\end{center}
\vspace*{1cm}
% -----------------------------------------------------


My sincere gratitude goes to my supervisor Alessandra. The example you have set will help me strive to become a great scientist in the future. I would also like to thank you for allowing me to develop my interests, for the advice and words of encouragement, and for providing us with an excellent research environment at the Albert Einstein Institute.

Thank you, Jon. Your approach to research has profoundly shaped my own. I am very glad you introduced me to the magical world of statistics! (*waves hands*). I hope that in this thesis I have given some justice to the work we have carried out in the last year of my PhD. I am very much looking forward to future collaborations. 

I want to thank Harald  for readily agreeing to be my second supervisor. I have learnt a great deal from you, both from a technical standpoint and by observing you interact with students in your course. Your advice has always been valuable and appreciated. 

Thank you Jean-Luc for kindly agreeing to be my mentor, and for always sharing kind words over coffee or casual conversations.

The work in this manuscript has been greatly influenced by three legendary figures of the AEI: Jan, Justin and Maarten. Thank you for teaching me the basics of how research is done, how to ask the right questions, as well as methods and techniques that I have used and will use in my research works. I also want to thank my collaborators in several other (published and unpublished) projects: Riccardo, Chris, Mohammed, Stefano, Laura, Lorenzo S., Nicola.
Everyday I keep learning from from you. I have enjoyed every single interaction I have had, and I am sure there will be many more in the years to come.

I want to single out my collaborator $\Gamma_{ij}$ (Ollie, the Fisher matrix guy). You have been a companion in (mis)fortune in the last year of PhD. It is fair to say all the practical knowledge on gravitational-wave data analysis I have traces back to you.  I have enjoyed our collaboration, and I am happy we have published at least one work together during the PhD. I am looking forward to more years of collaboration, projects, and all-around banter.

For the great time I have spent at the AEI I want to thank my fellow PhD students (in random order): Roberto, Hannes ($\times$2), Hugo, the trinity of Lorenzos (C., P., and S.), Łukas Prudensky, Mohammed, \footnote{Nils}, \footnote{Riccardo}, Niko, Noah, $\Gamma_{ij}$, Saketh. Thank you also to all the postdocs (too many to list here!), Darya for helping us international students navigate the meanders of German bureaucracy, and Brit and Matthias for the help throughout the years.

Part of the writing of this thesis coincided with several sporting occasions that have distracted me in times when distractions from writing were sorely needed. For the everlasting memories, I want to thank: Gigio Donnarumma, Giorgio Chiellini, Jorginho, Federico Chiesa, Lorenzo Insigne, Roberto Mancini, Gimbo Tamberi, Lamont Marcell Jacobs, Filippo Tortu, Fausto Desalu, Lorenzo Patta, and Filippo Ganna. 
These memorable moments would have not been the same without the presence of lifelong friends: Brus, Fede Ombres, Giulio, Lingio and Lollo. 

La mia esperienza di dottorando in Germania, così come precedentemente quella di studente in Inghilterra, non avrebbe potuto essere il successo che credo sia stato senza il supporto incondizionato dei miei genitori, Anna e Marcello. Vi sarò sempre grato per le possibilità che mi avete dato.
\newline

\emph{Finally, I dedicate this thesis to my dogs Boris and Momo, the most loyal companions one could wish for. }



==> intro/introduction.tex <==
%******************************************************
%*    LaTex-Vorlage für wissenschaftliche Arbeiten    *
%*    --------------------------------------------    *
%*      Autor: Jan Brennenstuhl (@jbspeakr)           *
%*             www.funkblocka.de                      *
%*            Lizenz: CC BY-SA 3.0                    *
%******************************************************
\begin{large}

\vspace*{2cm}
\noindent
Ich versichere, dass ich die von mir vorgelegte Arbeit selbstständig verfasst habe, dass ich die verwendeten Quellen, Internet-Quellen und Hilfsmittel vollständig angegeben habe und dass ich die Stellen der Arbeit - einschließlich Tabellen, Karten und Abbildungen -, die anderen Werken oder dem Internet im Wortlaut oder dem Sinn nach entnommen sind, in jedem Fall unter Angabe der Quelle als Entlehnung kenntlich gemacht habe.\vspace{2cm}

\noindent
Potsdam, den X. Month 2021

\vspace{3cm}

\hspace*{6cm}%
\dotfill\\
\hspace*{7cm}%
\textit{(Unterschrift des Kandidaten)}

\end{large}


==> sections/0-preface.tex <==
%******************************************************
%*    LaTex-Vorlage für wissenschaftliche Arbeiten    *
%*    --------------------------------------------    *
%*      Autor: Jan Brennenstuhl (@jbspeakr)           *
%*             www.funkblocka.de                      *
%*            Lizenz: CC BY-SA 3.0                    *
%******************************************************


\newcommand{\refs}{\, {\color{red}[Refs]\, }}


\chapter*{Preface}
\label{sec:GWhist}

The abundance of recent binary black-hole and neutron-star detections following the iconic detection of GW150914\refs tempts us to think that gravitational-wave (GW) astrophysics is a young and booming field. While this is true from the point of view of the astrophysics that we can learn with GWs, it is not quite right from the theoretical viewpoint. Gravitational-wave theory is in fact a mature field with a long gestation of more than a hundred years that is currently enjoying a Reinassance period. 

Soon after Einstein penned down his famous equations in 1915\refs, the prospect of the mere existence of GWs rose to prominence as an idealised scenario to test their inner workings. Caught within the analogy with electromagnetic waves suggesting their existence, and the absence of dipolar emission in gravity seemingly negating it, GWs were regarded at times as an artifact of gauge freedom\footnote{Eddington, ``speed of thought''. Ref. to book.} and at times as a real entity, possibly even detectable! 
With the pendulum of GW theory swinging between these two possibilities, arguments for the existence of GWs were first made\refs, then retracted\refs, then counter-retracted\refs by Einstein and collaborators, while proponents of the existence of GWs and of their inexistence entrenched themselves for a battle of thoughts (the ``quadrupole controversy'') that would last for the better part of the century\refs.

Slowly but steadily, it became clear that not only GWs do indeed exist, but that they also carry away energy with them\footnote{The first person to be credited this discovery is the omnipresent Feynman, with his ''beeding stick'' analogy later expounded upon by Bondi\refs.}, which prompted Weber to search GWs directly, for the first time ever\refs. Any further doubts on the existence and detectability of GWs were dispelled with the Nobel-prize worthy radio observation of the Hulse-Taylor pulsar PSR B1913+16\refs. This pulsar and its neutron-star companion continuously lose orbital energy, leading to an observable decay in their orbital period. The decay was found to match with exquisite accuracy the prediction from emission due to GWs, indirectly confirming their existence.

While the indirect detection of GWs essentially ended the ``quadrupole controversy'', the battle of thoughts it had led to set in motion the machinery needed to \emph{directly} measure GWs and the properties of the compact objects generating them. This is a formidable technical challenge, since gravity only couples weakly to matter, thus leaving only a small imprint on a detector. Despite the challenges, already in 1972 Weiss proposed a concept for a laser interferometer\refs that is nothing short of visionary for a modern reader. The concept and analysis of potential noise sources forms the basis for the two detectors (Hanford in the state of Washington and Livingston in Lousiana) composing the Laser Interferometry Gravitational-wave Observatory (LIGO), the Virgo detector in Cascina, near Pisa and the Kagra detector in Japan\refs. In a laser interferometer, GWs pass by lasers shot along two L-shaped arms of $\sim4$ kms each. This leaves energy in the detector, which in turn distorts the laser ever so slightly (by an amount shorter than the radius of an atom), modulating the photons received by a photocounter: this allows us to ``see'' GWs. 

The long technical process that throughout the 70's, 80's, 90's and early 2000's led to the development of the infrastructure needed for the LIGO interferometer bore its fruits on September 14th, 2015, when the two detectors (almost) concurrently detected the GWs from a binary black hole. This event marks a turning point in GW astronomy, rightfully vindicating the ``astronomy'' in its name, as well as for astrophysics in general. After the first detection, the Virgo detector joined the network\refs, playing a crucial role of the first detection of a binary neutron star in 2017. This event is credited for the birth of multimessenger astrophysics, as the same binary was seen by GWs and all bands of the electromagnetic spectrum\refs. As the sensitivity of the network increased between observation runs, the detectors were also able to detect 48 other events (and counting). This marks another important paradigm shift in which the full set of GW events can be used to begin answering questions regarding the formation channels leading to the observed black holes\refs, or to measure quantities of interest for Cosmology (such as the Hubble constant\refs). It is expected that the next few years will continue providing previously unaccessible (or even unthinkable) information on the darkest recesses of our Universe.

The successes of GW astrophysics have not gone unnoticed, garnering interest from communities that have been historically distant from classical physics and the general theory of relativity that most clearly symbolises its successes. This is the case for GW theory, which has enjoyed a Reinassance period in which tools and techniques from particle physics have been applied to the classical motion of compact objects, as required by the LIGO-Virgo observations. Such is the perimeter in which the work I present in this thesis mostly lies. In Sec.XX, I discuss these techniques -- known as \emph{scattering-amplitude} techniques, and how we can use them for the purposes of waveform modelling of compact-object coalescences. Section 2 is a publication in which we show that indeed this information can be used to directly inform waveform templates used in LIGO-Virgo analyses, even though current information is not enough to improve on them. Sections 4 and 5 are publications in which we show that theoretical advances that are intimately linked to these new computational techniques can be already used to indirectly improve on LIGO-Virgo templates. It is also importnt to mention that the flurry of activity in GW theory has not been limited to the above-mentioned scattering-amplitude techniques. The constant need for improvements in analytical predictions has led to a re-think of the analytical bases of waveform templates. I present a clear case of this in Sec.~3, where a model based on black-hole perturbation theory (rather than the weak-field, small-velocities) post-Newtonian approximation is presented.

The future of GW astrophysics is undoubtedly bright. While the current network of detectors reshapes the landscape of astrophysics, preparations are being made for future detectors both on the ground\refs and in space, with the Laser Interferometer Space Antenna (LISA). These detectors promise thousands if not millions of sources, presenting both an exciting astrophysical prospect and a unique set of challenges. Among the biggest challenges there is the question of how to simultaneously infer from an unkwown number of sources. In Sec.6, I present how this is a problem by showing what kind of biases one gets when a host of unknown sources have either gone missing in the data stream, or are incorrectly fitted out from it. 


The present thesis is organized as follows.
 
\begin{itemize}
	\item add contributions.
	\item add style choices.
\end{itemize}

\endinput 
